SpectralZoom: Efficient Segmentation with an Adaptive Hyperspectral Camera

Hyperspectral image segmentation is crucial for many fields such as agriculture, remote sensing, biomedical imaging, battlefield sensing and astronomy. However, the challenge of hyper and multi spectral imaging is its large data footprint. We propose both a novel camera design and a vision transformer-based (ViT) algorithm that alleviate both the captured data footprint and the computational load for hyperspectral segmentation. Our camera is able to adaptively sample image regions or patches at different resolutions, instead of capturing the entire hyperspectral cube at one high resolution. Our segmentation algorithm works in concert with the camera, applying ViT-based segmentation only to adaptively selected patches. We show results both in simulation and on a real hardware platform demonstrating both accurate segmentation results and reduced computational burden.

==> fig/hard_results.tex <==
\begin{figure*}[h]
\centering

\subfloat[Input image]{\includegraphics[width=0.3\linewidth]{Attachments/hard results/base.png}}\imghspace
\subfloat[Close up on patches]{\includegraphics[width=0.3\linewidth]{Attachments/hard results/zooms.png}}\imghspace
\subfloat[Segmentations]{\includegraphics[width=0.3\linewidth]{Attachments/hard results/segs.png}}\imghspace
\caption{Fully implemented imaging results. High resolution patches have been superimposed on the low resolution scene simulating what the network would see. The segmentation identifies the sky and treeline in the background along with several cars. }
\label{fig:hard results}
\end{figure*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


